Incentivized Bandit Learning with Self-Reinforcing User Preferences

In this paper, we investigate a new multi-armed bandit (MAB) online learning model that considers real-world phenomena in many recommender systems: (i) the learning agent cannot pull the arms by itself and thus has to offer rewards to users to incentivize arm-pulling indirectly; and (ii) if users with specific arm preferences are well rewarded, they induce a "self-reinforcing" effect in the sense that they will attract more users of similar arm preferences. Besides addressing the tradeoff of exploration and exploitation, another key feature of this new MAB model is to balance reward and incentivizing payment. The goal of the agent is to maximize the total reward over a fixed time horizon $T$ with a low total payment. Our contributions in this paper are two-fold: (i) We propose a new MAB model with random arm selection that considers the relationship of users' self-reinforcing preferences and incentives; and (ii) We leverage the properties of a multi-color Polya urn with nonlinear feedback model to propose two MAB policies termed "At-Least-$n$ Explore-Then-Commit" and "UCB-List". We prove that both policies achieve $O(log T)$ expected regret with $O(log T)$ expected payment over a time horizon $T$. We conduct numerical simulations to demonstrate and verify the performances of these two policies and study their robustness under various settings.

==> Sec1_Introduction/Introduction__Zhou_Tianchen_s_conflicted_copy_2021-01-30_.tex <==
%%%%%%%% ICML 2021 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:introduction}

In many online learning systems, there exists a self-reinforcing phenomenon, where the current user's behavior is influenced by the user behaviors in the past \citep{barabasi1999emergence, chakrabarti2005influence, ratkiewicz2010characterizing}, or an item is getting increasingly more popular as it accumulates more positive feedbacks.
%This can make future players lean to some item that originally has large bias but does not maximize total profit in the long run, which leads to sub-optimal result.
For example, on a movie rental website, current customers tend to have more interest in Movie A that has $500$ positive reviews, compared with Movie B that only has $10$ positive reviews.
On the other hand, the website owner, who aims to maximize the total profit in the long run, wants to identify the most profitable movies.
The online learning problem under self-reinforcing preferences can be modeled by the multi-armed bandit (MAB) framework \citep{berry1985bandit, bubeck2012regret}.
In the classic stochastic MAB setting, an agent observes and chooses to pull an arm (action).
The chosen arm, as feedback, generates a random reward from an unknown distribution and is assumed to be independent and identically distributed (i.i.d.) over time.
The agent, aiming to maximize total rewards over a given time horizon $T$, tries to design a strategy to perform arm selection in the presence of unknown arm reward distributions.

In the literature, existing works \citep{fiez2018multi, shah2018bandit} that incorporate the self-reinforcing preferences into the MAB model remain limited.
\citet{shah2018bandit} showed that the self-reinforcing preferences might render the classic UCB (upper confidence bound) algorithm \citep{auer2002finite} sub-optimal, and proposed new optimal arm selection algorithms.
However, in many online recommender platforms that utilize the MAB framework for online sequential decision making (e.g., recommender systems, healthcare, finance, and dynamic pricing, see \citep{bouneffouf2019survey}), the learning agent (i.e., a service provider) cannot select arms directly.
Rather, arms are pulled by users who are exhibiting self-reinforcing preferences.
The agent thus needs to incentivize users to select certain arms to maximize the total rewards, while avoiding incurring high incentive costs.
Hence, the bandit models in \citep{fiez2018multi, shah2018bandit} are no longer applicable even though the self-reinforcing preferences behavior is considered.
On the other hand, there exist several works \citep{frazier2014incentivizing, mansour2015bayesian, mansour2016bayesian, wang2018multi} that studied incentivized bandit under various settings and proposed efficient algorithms (more details in Section \ref{sec:related works}), but none of these works models users with self-reinforcing preferences.
To our knowledge, our work is the {\em first} to jointly consider both incentives and self-reinforcing preferences in the MAB framework -- two key features of many online learning systems in practice.
Moreover, we note that the joint consideration of incentives and self-reinforcing user preferences is {\em not} a trivial integration and its combined effect creates significant challenges in analyzing this new MAB model, which necessitates the use of new analytical techniques for MAB policy design.

Specifically, in this paper,
%in this paper, we express the relationship of user preferences and incentive by random arm selections.
%To our knowledge, most existing works, regarding either incentivizing bandits or MAB with user preferences, have a strong assumption of deterministic users pulling arms greedily or foreseeably.
%This is apparently not realistic in most e-Commerce platforms since user behaviors are random and unpredictable.
we first propose a more general MAB model with stochastic arm selections following user preferences, which is closely modeling random user behaviors in most online recommender systems.
This is in stark contrast to most existing works in the areas of incentivized bandits \citep{shah2018bandit}, where a (unrealistic) deterministic greedy user behavior is often assumed.
%we propose a new MAB model to address the self-reinforcing preferences and incentivized arm selections.
Under this model, two fundamental trade-offs naturally emerge: On the one hand, sufficient exploration is required to identify an optimal arm, which may result in multiple pullings of sub-optimal arms, while adequate exploitation is needed to stick with the arm that did well in the past, which may or may not be the best choice in the long run.
On the other hand, the agent needs to provide enough incentives to mitigate unfavorable self-reinforcing user preferences (i.e., initial biased crowd may attract more users of the same type), while in the meantime avoiding unnecessarily high compensations for users.
As in most online learning problems, we use \textit{regret} as a benchmark to evaluate the performance of our MAB policy, which is defined as the performance gap between the proposed policy and an optimal policy in hindsight. 
The major challenges thus lie in the following fundamental questions: 
\vspace{-.1in}
\begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=.0em}
\item[(a)] During incentivized pulling, how could the agent maintain a good balance between exploration and exploitation so as to minimize regret?
%keep a balance between exploration to seek an optimal arm and exploitation to maximize the current total reward.

\item[(b)] How long should the agent incentivize until the right self-reinforcing user preference is established toward an optimal arm, so that no further incentive is needed?
%with overwhelming probability.

\item[(c)] Is the established self-reinforcing user preferences sufficiently strong and stable to sustain the sampling of an optimal arm over time without additional incentives? 
If yes, under what conditions could this happen?
\end{list}
%Thus the major problem we want to study is the trade-off: by offering payment the controller is able to do enough exploration to maximize accumulative reward in the long run, while the controller also want to save payment as much as possible.\\

\vspace{-.1in}
In this work, we address the above challenges by proposing two ``$\log(T)$-regret-with-$\log(T)$-payment'' policies for the incentivized MAB framework with self-reinforcing preferences.
Our contributions are summarized as follows:
\vspace{-.1in}
\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=-0.0em \itemsep=-.2em}
%  \item We propose an incentivized bandit learning model with nonlinear feedback.
%  Compared to the basic stochastic MAB model, this proposed model considers non-deterministic pulling from users who exhibit self-reinforcing preferences, and the service provider implements a bandit policy with incentives.
%%  Specifically, the current preferences are formulated by a nonlinear function $F$ with parameter $\alpha$ catching the strength of the history impact.
%%  For each time step, the controller offers a constant payment on its favorable arm to incentivize pulling.
%%  As a result of the payment, the current player exhibits increased preference on the arm favored by the controller.
%%\textcolor{brown}{\sout{The impact of incentivizing on the preference distributions over arms is captured by a coefficient.}}
%  To our knowledge, this is the first work that integrates both self-reinforcing preference and incentive in MAB.
\item We first show that no incentivized bandit policy can achieve a sub-linear regret with a sub-linear total payment if the feedback function that models the self-reinforcing preferences has a super-polynomial growth rate.
The proof is inspired by a multi-color P\'{o}lya urn model, and we also show how to guide the self-reinforcing preferences toward a desired direction.

\item We propose two bandit policies, namely At-Least-$n$ Explore-Then-Commit (ETC) and UCB-List, both of which are optimal in regret.
Specifically, for the two policies, we analyze the upper bounds of the expected regret and the expected total payment over a fixed time horizon $T$.
We show that both policies achieve $O(\log T)$ expected regrets, which meet the lower bound in \citet{lai1985asymptotically}.
Meanwhile, the expected total incentives for both policies are upper bounded by $O(\log T)$.

\item We note that our MAB policies are {\em not} straightforward adoptions of ETC and UCB approaches. 
To address the dilemma between incentive costs and inducing favorable self-reinforcing user preferences, 
our {\em three-phase MAB policy architecture} and our key idea to show an $O(\log T)$ incentivizing period being sufficient for establishing {\em dominance} for the multi-color P\'{o}lya urn model (see Section~\ref{sec:policies}) are all new in the literature, which could be of independent interest for general incentivized MAB problems.

%\item We conduct extensive simulations to demonstrate the performance of both policies.
%Our results show that both policies are not only effective in performance but also insensitive to various parameter settings.
%  \sout{The simulations also reveal the trade-off between exploration and exploitation during incentivized pulling, which is controllable by tuning parameters of At-Least-$n$ Greedy and UCB-List.}
  \end{list}



% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021. Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.


==> Sec1_Introduction/Introduction__Zhou_Tianchen_s_conflicted_copy_2021-02-01_.tex <==
% !TEX root = ../incentive_MAB.tex

\section{Introduction}\label{introduction}

In many online e-Commerce platforms, there exists a self-reinforcing phenomenon, where the current user's behavior is influenced by the user behaviors in the past \citep{barabasi1999emergence, chakrabarti2005influence, ratkiewicz2010characterizing}, or an item is getting increasingly more popular as it accumulates more positive feedbacks.
%This can make future players lean to some item that originally has large bias but does not maximize total profit in the long run, which leads to sub-optimal result.
For example, on a movie rental website, current customers tend to have more interest in Movie A that has $500$ positive reviews, compared with Movie B that only has $10$ positive reviews.
As an online learner, the e-Commerce service provider wants to identify the most profitable item in order to maximize the total profit in the long run.
In the literature, such an online profit maximization problem can often be modeled by the multi-armed bandit (MAB) framework \citep{berry1985bandit, bubeck2012regret}.
%As in the classic stochastic MAB setting, a learning agent observes and chooses to pull an arm (action).
%The chosen arm, as feedback, generates a random reward from an unknown distribution and is assumed to be independent and identically distributed (i.i.d.) over time.
%The agent, aiming to maximize total rewards over a given time horizon $T$, tries to design a strategy to perform arm selection in the presence of unknown arm reward distributions.
However, existing works on MAB that consider the self-reinforcing preferences remain quite limited (see, e.g., \citep{fiez2018multi, shah2018bandit}).
In fact, \citet{shah2018bandit} showed that the self-reinforcing preferences might render the classic UCB (upper confidence bound) policy \citep{auer2002finite} sub-optimal, and  new optimal arm selection algorithms are necessary.

On the other hand, in many online learning problems that utilize the MAB framework for  sequential decision making (e.g., recommender systems, healthcare, finance, dynamic pricing, see \citep{bouneffouf2019survey}), the learning agent (e.g., an online service provider) {\em cannot} select the arms directly.
Rather, arms are pulled by the users who are exhibiting self-reinforcing preferences.
The agent thus needs to {\em incentivize} users to select certain arms to maximize the total rewards, while avoiding incurring high incentive costs.
Hence, the bandit models in \citep{fiez2018multi, shah2018bandit} are no longer applicable, even though the self-reinforcing preferences behavior is considered.
Meanwhile, there exist several works \citep{frazier2014incentivizing, mansour2015bayesian, mansour2016bayesian, wang2018multi} that studied incentivized bandit under various settings and proposed efficient algorithms (more details in Section \ref{sec:related works}), but none of these works models users with self-reinforcing preferences.

The missing of joint modeling of incentives and self-reinforcing preferences in the existing MAB framework (two key features of many online e-Commerce systems) motivates us to fill this gap in this paper.
%To our knowledge, our work is the {\em first} to jointly consider both .
%Moreover, we note that the joint consideration of incentives and self-reinforcing user preferences is {\em not} a trivial integration and its combined effect creates significant challenges in analyzing this new MAB model, which necessitates the use of new analytical techniques for MAB policy design.
Specifically, in this work,
%in this paper, we express the relationship of user preferences and incentive by random arm selections.
%To our knowledge, most existing works, regarding either incentivizing bandits or MAB with user preferences, have a strong assumption of deterministic users pulling arms greedily or foreseeably.
%This is apparently not realistic in most e-Commerce platforms since user behaviors are random and unpredictable.
we first propose a more general MAB model with {\em stochastic arm selections following user preferences}, which is closely modeling random user behaviors in most online recommender systems.
This is in stark contrast to most existing works in the areas of incentivized bandits \citep{shah2018bandit}, where a (unrealistic) deterministic greedy user behavior is often assumed.
%we propose a new MAB model to address the self-reinforcing preferences and incentivized arm selections.
Under this model, a pair of fundamental trade-offs naturally emerge: (1) Sufficient exploration is required to identify an optimal arm, which may result in multiple pullings of sub-optimal arms, while adequate exploitation is needed to stick with the arm that did well in the past, which may or may not be the best choice in the long run;
(2) The agent needs to provide enough incentives to mitigate unfavorable initial bias and self-reinforcing user preferences, while in the meantime avoiding unnecessarily high incentives for users.
As in most online learning problems, we use regret as a benchmark to evaluate the performance of our MAB policy, which is defined as the performance gap between the proposed policy and an optimal policy in hindsight. 
The major challenges in this new MAB model thus lie in the following fundamental questions: 
\vspace{-.1in}
\begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=.0em}
\item[(a)] During incentivized pulling, how could the agent maintain a good balance between exploration and exploitation to minimize regret?
%keep a balance between exploration to seek an optimal arm and exploitation to maximize the current total reward.

\item[(b)] How long should the agent incentivize until the right self-reinforcing user preference is established toward an optimal arm (so that no further incentive is needed)?
%with overwhelming probability.

\item[(c)] Is the established self-reinforcing user preferences sufficiently strong and stable to sustain the sampling of an optimal arm over time without additional incentives? 
If yes, under what conditions could this happen?
\end{list}
%Thus the major problem we want to study is the trade-off: by offering payment the controller is able to do enough exploration to maximize accumulative reward in the long run, while the controller also want to save payment as much as possible.\\

\vspace{-.1in}
In this work, we answer the above questions by proposing two ``$\log(T)$-regret-with-$\log(T)$-payment'' policies for the incentivized MAB framework with self-reinforcing preferences.
Our contributions are summarized as follows:
\vspace{-.1in}
\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=-0.0em \itemsep=-.2em}
%  \item We propose an incentivized bandit learning model with nonlinear feedback.
%  Compared to the basic stochastic MAB model, this proposed model considers non-deterministic pulling from users who exhibit self-reinforcing preferences, and the service provider implements a bandit policy with incentives.
%%  Specifically, the current preferences are formulated by a nonlinear function $F$ with parameter $\alpha$ catching the strength of the history impact.
%%  For each time step, the controller offers a constant payment on its favorable arm to incentivize pulling.
%%  As a result of the payment, the current player exhibits increased preference on the arm favored by the controller.
%%\textcolor{brown}{\sout{The impact of incentivizing on the preference distributions over arms is captured by a coefficient.}}
%  To our knowledge, this is the first work that integrates both self-reinforcing preference and incentive in MAB.
\item We first show that no incentivized bandit policy can achieve a sub-linear regret with a sub-linear total payment if the feedback function that models the self-reinforcing preferences has a super-polynomial growth rate.
The proof is inspired by a multi-color P\'{o}lya urn model, and we also show how to guide the self-reinforcing preferences toward a desired direction.

\item We propose two bandit policies, namely At-Least-$n$ Explore-Then-Commit (ALnETC) and UCB-List, both of which are optimal in regret.
Specifically, for the two policies, we analyze the upper bounds of the expected regret and the expected total payment over a fixed time horizon $T$.
We show that both policies achieve $O(\log T)$ expected regrets, which meet the lower bound in \citet{lai1985asymptotically}.
Meanwhile, the expected total incentives for both policies are upper bounded by $O(\log T)$.

\item Although based on ETC and UCB strategies, our proposed policies are {\em not} straightforward adoptions of these classical MAB approaches. 
To address the above challenges in the new MAB model, we propose (i) a {\em three-phase MAB policy architecture} and (ii) a key idea showing that an $O(\log T)$ incentivizing period is sufficient for establishing {\em dominance} for the multi-color P\'{o}lya urn model (see Section~\ref{sec:policies}).
All of these results are new in the bandit literature, which could be of independent interest for general incentivized MAB problems.

%\item We conduct extensive simulations to demonstrate the performance of both policies.
%Our results show that both policies are not only effective in performance but also insensitive to various parameter settings.
%  \sout{The simulations also reveal the trade-off between exploration and exploitation during incentivized pulling, which is controllable by tuning parameters of At-Least-$n$ Greedy and UCB-List.}
  \end{list}



% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021. Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.


==> Sec4_Policies/Policies__Zhou_Tianchen_s_conflicted_copy_2021-01-30_.tex <==
%%%%%%%% ICML 2021 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%

\section{Policies and Upper Bounds}\label{sec:policies}

In this section, we present two policies that achieve $O(\log T)$ expected regret with $O(\log T)$ accumulative payment with respect to time horizon $T$.
The main ideas of these two policies are similar: we first perform exploration among all arms by incentivizing pulling until we know the best-empirical arm is optimal, i.e., $\hat a^* = a^*$ with high confidence; then, we keep incentivizing the pulling of the best-empirical arm $\hat a^*$ until it dominates.
To this end, we formally define the notion of dominance as follows: 
\begin{definition}[Dominance] \label{defn_dominance}
An arm is said to be dominant if it produces at least half of the total reward.
\end{definition}
%{\color{blue}
The key of the policies is to guarantee the dominance of arm $\hat a^*$, which induces the correct preference to arm $\hat a^*$, while keeping the accumulative payment sub-linear.
%}

Before presenting the policies, we want to show that if the feedback function $F(x)$ satisfies certain conditions, then with probability one, the users' self-reinforcing preferences converge to one arm without incentive after sufficiently many time steps, i.e., an arm $a\in A$ is the only arm to be sampled.
We define this event as the \textit{monopoly by arm $a$}, or $mono_a$ for short.
We then define an incentivized policy as a policy that incentivizes pulling with bounded payment for a continuous duration smaller than or equal to time horizon $T$. 
Clearly, monopoly is necessary for the existence of an incentivized policy that induces all users' preferences to a certain arm with sub-linear total payment.
Correspondingly, if such a policy exists, then it implies that the system enjoys the property that the users' self-reinforcing preferences converge to a certain arm even after the service provider stops providing incentives at some stage.

\begin{restatable}{lemma}{RestateLEMMA}{\em (Monopoly)}
\label{prop}
There exists an incentivized policy that induces users' preferences to converge in probability to an arm over time with sub-linear payment, if and only if $F(x)$ satisfies $\sum_{i=1}^{+\infty}\big(1/F(i)\big)<+\infty$.
\end{restatable}

\begin{proof}[Proof Sketch]
Our main mathematical tool is the improved exponential embedding method.
In a nutshell, this method simulates the reward generating sequence by random exponentials.

\textbf{Problem clarification.} Define a sequence $\lbrace\chi_j\rbrace_{j=1}^\infty$ denoting the reward generating order, where each element denotes the arm index.
Note that an arm index appears in $\lbrace\chi_j\rbrace$ only when it is pulled and generates a unit reward.
We want to construct a sequence $\lbrace \zeta_j\rbrace$ that has the same conditional distribution as $\lbrace\chi_j\rbrace$ given history $\mathcal{F}_{j-1}$.
Then the constructed sequence $\lbrace \zeta_j\rbrace$ is leveraged to prove the lemma.

\textbf{Construction of reward generating sequence.} For arm $i\in A$, consider a collection of independent exponential random variables $\lbrace r_i(n)\rbrace$ such that $\mathbb{E}[r_i(n)]=1/[\mu_iF(n+\theta_i)]$.
We construct an infinite set $B_i=\lbrace\sum_{k=0}^nr_i(k)\rbrace_{n=0}^\infty$, where each element $\sum_{k=0}^nr_i(k)$ models the time needed for arm $i$ to get $n$ accumulative rewards.
Then we mix up and increasingly sort $B_i$ for all $i\in A$ to form a new sequence $H$.
Our objective sequence $\lbrace \zeta_j\rbrace$ is the arm index sequence out of $H$.
Next, we prove by induction that given the previous reward history $\mathcal{F}_{j-1}$, the constructed sequence $\lbrace \zeta_j\rbrace$ has the same conditional distribution as $\lbrace\chi_j\rbrace$.

Then, \textbf{the proof of Lemma~\ref{prop}} is done if we show that if and only if any feedback function $F(x)>0$ satisfies $\sum_i \big(1/F(i)\big)<+\infty$, then $\mathbb{P}(\exists a\in A,\, mono_a)=1$.
We define the \textit{attraction time} $N$ as the time step when the monopoly happens.
With the constructed sequence $\lbrace \zeta_j\rbrace$, we establish the necessity by showing that if $\sum_i \big(1/F(i)\big)<+\infty$ then $\mathbb{P}(N<\infty)=1$, and the sufficiency by showing that if $\sum_i \big(1/F(i)\big)=+\infty$ then $\mathbb{P}(N=\infty)>0$.
\end{proof}


\begin{remark}{\em
	The exponential embedding technique has been widely applied \citep{zhu2009nonlinear, oliveira2009onset, davis1990reinforced, athreya1968embedding}.
	This method embeds a discrete-time process into a continuous-time process built with exponential random variables.
	We improve this method and adapt it to our model, which considers more random variables.
	The most significant feature of the exponential embedding technique is that the random times of different arms generating unit rewards are independent and can be mathematically expressed with exponential distributions, which facilitates our subsequent analysis.}
\end{remark}

\begin{remark}{\em
	As a special case, if $F(x)=x^\alpha$ with $\alpha>1$ (i.e., superlinear polynomial), then there exists an incentivized policy that induces all preferences to converge over time with sub-linear total payment, since $\sum_{i=1}^{+\infty}(1/i^\alpha)<+\infty$ with $\alpha >1$.
	Previous works \citep{drinea2002balls,khanin2001probabilistic} considering the balls and bins model also studied the cases $\alpha<1$ and $\alpha=1$.
	In the case $\alpha<1$, the asymptotic preference rates of arms are all deterministic, positive, and dependent on the means and biases of arms.
	In the case $\alpha=1$, the system is akin to a standard P\'{o}lya urn model, and will converge to a state where all arms have random positive preference rates that depend on the means and initial biases of the arms.
	In the case $\alpha>1$, the system converges almost surely to a state where only one arm has a positive probability to generate rewards, depending on the means and initial biases of arms.
	Thus, the system under these three conditions exhibits completely different behaviors.}
\end{remark}






\subsection{Explore-Then-Commit}
The Explore-Then-Commit policy consists of three phases: the exploration phase, the exploitation phase, and the self-sustaining phase.
The service provider participates in the first two phases.
During the exploration phase, the Explore-Then-Commit policy explores all arms  until each arm generates sufficient accumulative rewards.
Then, the policy exploits the arm with the best empirical mean until it dominates (as defined in Definition~\ref{defn_dominance}).
%{\color{blue}
We show that once the best-empirical arm dominates, there is an overwhelming probability that after finite time steps in the self-sustaining phase, monopoly happens on the best-empirical arm, which implies sub-linear regret.
{\em One of our key contributions in this paper is the discovery} that the incentive can stop as soon as the dominance happens, which is much {\em earlier than} the monopoly established and guarantees sub-linear accumulative payment.
%}
In both policies, we define the sample mean of arm $a\in A$ at time step $t$ as $\hat\mu_a(t) = S_a(t-1)/T_a(t-1)$, and all ties broken at random.
The Explore-Then-Commit policy is stated as follows:

\begin{policy}[Explore-Then-Commit]
Given the time horizon $T$, payment $b$ and $n = q\log T$.

{\normalfont \textbf{1) Exploration Phase:}} 
Incentivize pulling arm $a\in \arg\min_{i\in A}S_i(t)$ with payment $b$ until time $\tau_n = \min\lbrace t: S_a(t)\geq n,\, \forall a\rbrace\land T$, when any arm has accumulative reward of at least $n$.
%Let $\tau_n = \min(t: S_a(t)\geq n,\, \forall a)\land T$ denote the random time step where any arm has accumulative reward of at least $n$.
%For $t\in [1, \tau_n]$, incentivize users with payment $b$ to sample arm $I(t)\in \arg\min\limits_{a\in A}S_a(t)$, with ties broken at random.

{\normalfont \textbf{2) Exploitation Phase:}}
Incentivize pulling the best-empirical arm $\hat a^*\in \arg\max_{a\in A}\hat\mu_a(\tau_n)$ with payment $b$ until it dominates: $S_{\hat a^*}(t)=\sum_{a\neq \hat a^*}S_a(t)$. Mark current time as $\tau_s$.
%Let $\hat a^* \in \arg\max\limits_{a\in A}\hat\mu_a(\tau_n+1)$, with ties broken at random.
%Let $\tau_s = \tau_n + \delta\tau_n$, where $\delta = {G(b)+1\over G(b)-1}$.
%For $t\in (\tau_n, \tau_s]$, the service provider offers payment $b$ for users to sample arm $\hat a^*$.

{\normalfont \textbf{3) Self-Sustaining Phase:}}
Users pull arms based on their own preferences until time $T$.
%For $t\in (\tau_s, T]$, the service provider stops offering payments and lets users sample arms based on their own preferences.
\end{policy}

\begin{restatable}{lemma}{RestateLEMMA}{\em (Dominance)}
\label{dominance}
If the sensitivity function $G(\cdot)$ and the payment $b$ satisfy $G(b)>1$, then the expected dominant time $\tau_s$ is $O(\log T)$.
\end{restatable}

Since with enough time steps after $\tau_s$, monopoly happens with probability one and arm $\hat a^*$ has high probability to emerge victorious in monopoly (to be shown in the proof of Theorem \ref{thm-etc}). 
If the time horizon $T$ is large enough to cover the attraction time, then arm $\hat a^*$ will be sampled repeatedly after monopoly happens, while the accumulative reward generated by sub-optimal empirical arms after the dominance is inversely proportional to $O(\log T)$  (which contribute to the regret).
%For each arm $a$, we set $\Delta_a=\mu^*-\mu_a$.
Thus, the policy achieves a sub-linear expected regret stated as follows:

\begin{restatable}{theorem}{RestateETC}{\em (Explore-Then-Commit)}
\label{thm-etc}
Given a fixed time horizon $T$.
If (i) $G(b)>1$, (ii) $q\geq (2\max_{a\neq a^*}\mu_a)/\Delta_{min}^2$, and (iii) $F(x)=\Theta(x^\alpha)$ with $\alpha>1$,
%(iii) $F(x)$ is in the range $\Omega(x^\alpha)$ and $O(x^\beta\ln x)$ with $\alpha,\beta>1$,
then the expected regret of the Explore-Then-Commit is
\begin{equation*}
	\mathbb{E}[R_T] \leq \sum\limits_{a\in A}\cfrac{2(G(b)-L_{a^*})\Delta_{max}}{\big(G(b)-1\big)\mu_a}\cdot q\log T + o(\log T),
\end{equation*}
where $L_a=F(q\log T+\theta_a)/\sum_{i\in A}F(\mu^*T+\theta_i)$, with the expected payment
\begin{equation*}
	\mathbb{E}[B_T]\leq\sum\limits_{a\neq a^*}\cfrac{2b(G(b)+1)}{\mu_a(G(b)-1)}\cdot q\log T.
\end{equation*}
%$\mathbb{E}[B_T]\leq\sum\limits_{a\neq a^*}\cfrac{2b(G(b)+1)}{\mu_a(G(b)-1)}\cdot q\log T$.
\end{restatable}

\begin{proof}[Proof Sketch]
By the law of total expectation, the expected regret up to time $T$ can be decomposed as
\begin{equation*}
	\mathbb{E}[R_T]\leq\underbrace{\mathbb{E}[R_T \mid\hat a^* = a^*]}_\text{(a)} + T\cdot\underbrace{\mathbb{P}(\hat a^*\neq a^*)}_\text{(b)}.
\end{equation*}
To bound $\mathbb{E}[R_T]$, we want to upper bound both $\mathbb{E}[R_T \mid\hat a^* = a^*]$ and $\mathbb{P}(\hat a^*\neq a^*)$.
First, in (b), the probability $\mathbb{P}(\hat a^*=a^*)\leq\mathbb{P}\big(\hat\mu_a(\tau_n)\geq \hat\mu_{a^*}(\tau_n)\big)$ is bounded by $O(T^{-1})$ by leveraging the Chernoff-Hoeffding bound.
Since
\begin{equation*}
	(a)=\mu^* T - \big( \mathbb{E}[\Gamma_{\tau_s}\mid\hat a^* = a^*] + \mathbb{E}[\Gamma_T-\Gamma_{\tau_s}\mid\hat a^* = a^*]\big),
\end{equation*}
where $\Gamma_t$ is the accumulative reward up to time $t$, we first need to upper bound $\mathbb{E}[\tau_n]$ and $\mathbb{E}[\tau_s]$.
Consider $\mathbb{E}[\tau_n]$, we show that the number of pulling of arm $a$ to get a unit reward is a geometric random variable with parameter larger than $\mu_aG(b)/\big(G(b)+1\big)$.
Then, for each arm $a\in A$ to obtain at least $n$ accumulative reward, the expected time needed is bounded by
\begin{equation*}
	\mathbb{E}[\tau_n] \leq \cfrac{G(b)+1}{G(b)}\cdot \sum_{i\in A}\cfrac{1}{\mu_i}\cdot q\log T.
\end{equation*}
For $\mathbb{E}[\tau_s]$, since $\tau_s$ is the earliest time for the system to reach dominance, $\tau_s$ satisfies the condition $\mu_{\hat a^*}\mathbb{E}[T_{\hat a^*}(t)] \geq \sum_{a\neq \hat a^*}\mu_a\mathbb{E}[T_a(t)]$.
With the bound of $\mathbb{E}[\tau_n]$, after loosing the inequality and rearrangement we obtain the upper bound as follows
\begin{equation*}
	\mathbb{E}[\tau_s] \leq \cfrac{G(b)+1}{G(b)-1}\cdot\sum_{a\neq a^*}\cfrac{2}{\mu_a}\cdot q\log T.
\end{equation*}
According to the policy, the expected accumulative payment $\mathbb{E}[B_T]$ can be bounded by $b\mathbb{E}[\tau_s]$ and part of the expected regret $\mathbb{E}[\Gamma_{\tau_s}\mid\hat a^* = a^*]$.

%{\color{blue}
The next challenge is to show whether the dominant arm has a large enough probability to ``win'' in monopoly during the self-sustaining phase.
We construct an event $D(u_0, n_0)$ to describe the following phenomenon: the fraction of accumulative reward from a weak arm increases over time, i.e., at time step $\tau_s$, there are $u_0n_0$ accumulative reward from the weak arm, with $n_0$ total reward and the fraction $u_0<1/2$.
Then at time step $t'\in (\tau_s,\, T]$, there are $un$ accumulative reward from the weak arm with the fraction $u>u_0$.
Note that $u_0n_0=O(\log T)$.
The probability of event $D(u_0, n_0)$ can be bounded as $\mathbb{P}\big(\exists n > n_0,\, D(u_0, n_0)\big) \leq e^{-(u_0n_0)^\gamma}=e^{-O(\log T)^\gamma}$ with constant $\gamma\in(0,1/4)$ using the improved exponential embedding method and a Chernoff-like bound developed in Lemma~7.
The upper bound of event $D(u_0, n_0)$ decreases as $u_0n_0$ increases monotonically over time.
Thus the arms that stay on the weak side for a long time have little chance to win back.

Now we bound the last part of regret $\mathbb{E}[R_T - R_{\tau_s}\mid \hat a^* = a^*]$.
After time $\tau_s$, a unit reward is generated by sub-optimal arms with probability upper bounded by $e^{-(u_0n_0)^\gamma}$, and then the next unit reward is also generated by sub-optimal arms with probability upper bounded by $e^{-(u_0n_0+1)^\gamma}$.
Thus
\begin{equation*}
	\mathbb{E}[R_T - R_{\tau_s}\mid \hat a^* = a^*]\leq e^{-(u_0n_0)^\gamma} + e^{-(u_0n_0+1)^\gamma} + \cdots,
\end{equation*}
with the summation on the right hand side bounded by $O\big((\log T)^{1-\gamma}e^{-(\log T)^\gamma}\big)$ and $\gamma\in(0,1/4)$.
\end{proof}



\subsection{UCB-List}
In this section, we propose a UCB-List policy to further improve the performance of the Explore-Then-Commit policy.
The UCB-List policy is similar to Explore-Then-Commit and also consists of three phases.
During the exploration phase, the service provider initially puts all arms in one set, and then makes arm selection in the set in a way similar to the standard UCB policy.
Meanwhile, it removes arms that are estimated to be sub-optimal, until only one arm is left in the set, which is viewed as the best-empirical arm.
Note that in this phase users can still pull any arm regardless of the set.
Then, the service provider incentivizes users to sample this arm until it dominates.
Compared to Explore-Then-Commit, UCB-List reduces the pulling times of sub-optimal arms during the exploration phase, while still balances the trade-off between exploration and exploitation.
For each arm $a$, we set $\Delta_a=\mu^*-\mu_a$.
Formally, the UCB-list policy is stated as follows:

\begin{policy}[UCB-List]
Given the time horizon $T$ and payment $b$.
Define the confidence interval of arm $a$ at time step $t$ as $c_a(t) = \sqrt{\ln T/2T_a(t)}$.

{\normalfont \textbf{Initialization:}} Incentivize pulling arms satisfying $T_a(t)=0$ with payment $b$ until $\min_{a\in A}T_a(t)=1$.
Let set $U = A$.

{\normalfont \textbf{1) Exploration Phase:}} While $|U|>1$, remove any arm $a$ satisfying $\hat\mu_a(t)+c_a(t) \leq \max_{i\neq a, i\in U}\big(\hat\mu_i(t)-c_i(t)\big)$ from $U$ if there is any, then incentivize pulling arm $a\in \arg\min_{i\in U}T_i(t)$ with payment $b$.
If $|U|=1$, let arm $\hat a^* = \lbrace a: a\in U\rbrace$ and mark current time as $\tau_1$.

{\normalfont \textbf{2) Exploitation Phase:}} Incentivize pulling arm $\hat a^*$ with payment $b$ until it dominates: $S_{\hat a^*}(t)=\sum_{a\neq \hat a^*}S_a(t)$. Mark current time as $\tau_s$.

{\normalfont \textbf{3) Self-Sustaining Phase:}}
Users pull arms based on their own preferences until time $T$.
\end{policy}

%\begin{theorem}
\begin{restatable}{theorem}{RestateUCB}{\em (UCB-List)}
\label{thm-ucb-list}
Given a fixed time horizon $T$, if $G(b)>1$, and $F(x)=\Theta(x^\alpha)$ with $\alpha>1$, then the expected regret of the UCB-List $\mathbb{E}[R_T]$ is upper bounded by
\begin{equation*}
	\sum\limits_{a\neq a^*}\hspace{-3pt}\bigg(\cfrac{8\Delta_a\big(G(b)-1\big)\hspace{-2pt}+\hspace{-2pt}8\mu_a}{\big(G(b)-1\big)\Delta_a^2}\cdot \log T + 4\Delta_a+\cfrac{4\mu_a}{G(b)-1}\bigg),
\end{equation*}
%$\mathbb{E}[R_T] \leq \sum\limits_{a\neq a^*,\, a\in A} (\cfrac{8}{\Delta_a}+\cfrac{\gamma_p\Delta_a}{G(b)-1} )\log T + O(1) + O(T^{-3})$,
%with a constant $\gamma_p$ dependent on the parameter $p$.
with the expected payment $\mathbb{E}[B_T]$ upper bounded by
\begin{equation*}
	\cfrac{2G(b)+1}{G(b)-1}\bigg[\cfrac{8b\log T}{\Delta_{min}^2}+\sum_{a\neq a^*}\bigg(\cfrac{8b\log T}{\Delta_a^2}+b\bigg)\bigg].
%	\cfrac{8b\log T}{\Delta_{max}^2}+\hspace{-12pt}\sum_{a:\mu_a>\mu_{min}}\hspace{-5pt}\cfrac{8G(b)b\log T}{\big(G(b)-1\big)(\mu_a-\max\limits_{\mu_i<\mu_a}\mu_i)^2}.
\end{equation*}
%$\mathbb{E}[B_T] \leq \cfrac{2\gamma_pG(b)}{G(b)-1}\log T$.
\end{restatable}


\begin{proof}[Proof Sketch]
The expected time needed for initialization can be proved upper bounded by $O(1)$ trivially.
Then by the law of total expectation, the expected regret up to time $T$ can be decomposed as:
\begin{align*}
	\mathbb{E}[R_T]\leq &\underbrace{\mathbb{E}[R_{\tau_1}]}_\textbf{(a)}+\underbrace{\mathbb{E}[R_{\tau_2}-R_{\tau_1}\mid \hat a^*=a^*]}_\textbf{(b)} \\
	&+\underbrace{\mathbb{E}[R_T-R_{\tau_2}\mid \hat a^*=a^*]}_\textbf{(c)}+\underbrace{T\cdot \mathbb{P}(\hat a^*\neq a^*)}_\textbf{(d)}.
\end{align*}
In what follows, we will bound the four terms on the right-hand-side one by one.

\textbf{(a)} In the exploration phase, since the regret results from the pulls of sub-optimal arms, the expected regret at time step $\tau_1$ can be written as $\mathbb{E}[R_{\tau_1}]=\sum_{a\neq a^*}\Delta_a\mathbb{E}[T_a(\tau_1)]$.
Thus, term \textbf{(a)} can be bounded if we upper bound $\mathbb{E}[T_a(\tau_1)]$ for each $a\in A$.
The proof is similar to that of the standard UCB policy except that we consider in addition the randomness of user behaviors under incentives, since there exists a positive probability for users to pull arms that are not incentivized.
This possibility causing regret can be bounded based on the fact that without incentive, the expected preference rate on one arm decreases monotonically.
Thus, for each arm $a\in A$, we obtain $\mathbb{E}[T_a(\tau_1)]\leq 8\ln T/\Delta_a^2+O(1)$.

\textbf{(b)} In the exploitation phase, the expected regret $\mathbb{E}[R_{\tau_2}-R_{\tau_1}\mid \hat a^*=a^*]$ is upper bounded by $O(\mathbb{E}[\tau_2-\tau_1])$.
We first bound $\mathbb{E}[\tau_1]$, which equals $\sum_{a\in A}\mathbb{E}[T_a(\tau_1)]$.
Observing the policy, an arm is expected to be eliminated when its upper confidence interval is smaller than the smallest lower confidence interval of the rest arms.
Thus in the case of two arms, the sub-optimal arm $a$ is expected to be eliminated when
\begin{equation*}
	\sqrt{\cfrac{2\ln t}{\mathbb{E}[T_a(t)]}} + \sqrt{\cfrac{2\ln t}{\mathbb{E}[T_{a^*}(t)]}} < \Delta_a,
\end{equation*}
and we obtain $\mathbb{E}[T_{a^*}(t)] > 8\ln t/\Delta_a^2$.
Extend the result to the case of more arms we get
\begin{equation*}
	\mathbb{E}[\tau_1] \leq \bigg(\cfrac{8}{\Delta_{max}^2} + \sum_{a:\mu_a>\mu_{min}}\cfrac{8}{(\mu_a-\max\limits_{\mu_i<\mu_a}\mu_i)^2}\bigg)\ln T.
\end{equation*}
Then similar to the proof of Explore-Then-Commit, we obtain the bound of term \textbf{(b)} and $\mathbb{E}[B_T]$.
Note that the choice of $\tau_2$ has the same analysis as in the proof of Theorem~\ref{thm-etc}.

\textbf{(c)} This term represents the expected regret from time $\tau_2$ to $T$.
Similar to the proof of Theorem~\ref{thm-etc}, the expected regret during this phase is bounded by $O\big((\log T)^{1-\gamma}e^{-(\log T)^\gamma}\big)$ with $\gamma\in(0,1/4)$.

\textbf{(d)} The probability $\mathbb{P}(\hat a^*\neq a^*)$ can be bounded by $O(T^{-4})$ using the bounds of $\mathbb{E}[T_a(\tau_1)]$ for $a\in A$ and the Chernoff-Hoeffding bound.

Combining steps \textbf{(a)}--\textbf{(d)} yields the result stated in the theorem and the proof is complete.
\end{proof}



